Causality and deceit: Do androids watch action movies?

We seek causes through science, religion, and in everyday life. We get excited when a big rock causes a big splash, and we get scared when it tumbles without a cause. But our causal cognition is usually biased. The 'why' is influenced by the 'who'. It is influenced by the 'self', and by 'others'. We share rituals, we watch action movies, and we influence each other to believe in the same causes. Human mind is packed with subjectivity because shared cognitive biases bring us together. But they also make us vulnerable. An artificial mind is deemed to be more objective than the human mind. After many years of science-fiction fantasies about even-minded androids, they are now sold as personal or expert assistants, as brand advocates, as policy or candidate supporters, as network influencers. Artificial agents have been stunningly successful in disseminating artificial causal beliefs among humans. As malicious artificial agents continue to manipulate human cognitive biases, and deceive human communities into ostensive but expansive causal illusions, the hope for defending us has been vested into developing benevolent artificial agents, tasked with preventing and mitigating cognitive distortions inflicted upon us by their malicious cousins. Can the distortions of human causal cognition be corrected on a more solid foundation of artificial causal cognition? In the present paper, we study a simple model of causal cognition, viewed as a quest for causal models. We show that, under very mild and hard to avoid assumptions, there are always self-confirming causal models, which perpetrate self-deception, and seem to preclude a royal road to objectivity.

==> 6-cogsci-complex.tex <==
% !TEX root = 0-cogsci.tex

\subsection{Extensional explanations}

If only causes and effects are taken into account, then nothing about explanations is decidable.

ANDROIDS MUST TAKE THE SIMPLEST EXPLANATIONS. They must ask: WHO SPEAKS?




\subsection{OLD: Computational consequences of evolution: Logical depth}
**** selection according to behaviors is undecidable
**** where decisions are needed
**** genes are not transferred not just horizontally (hypersex) but split into genomes
**** that is why horizontal gene transfer got obstructed

\subsubsection{Church-Turing Antithesis} EVOLUTION INTO EUCARIOTS IS INTENSIONAL SELECTION, NOT BEHAVIORAL

34. MSRS Thm: TT is finitely approximable
**** open ended selection according to behaviors

35. ORACLES: 
** layered language generation: 
**** words: a-machines --- arbitrary!
**** sentences: a-machines or FSM --- simple, with stack memory
**** messages: o-machines --- feedback from conversation
**** protocols: o-machines --- extensive oracle interactions, run in parallel
**** contexts, narratives, experience, identity --- o-interactions, complexity degrees

36. ACTOR LOGIC

\subsubsection{High-level programming language for foundations}
Resumptions.

Complexity.




\subsection{Complexity bounding: MDL, Occam}
Only observations pump complexity into scientific theories. The wrong theory of Mercury's orbit is simpler than the correct one.

The natural gravity of logic, the quest for the truth, is NOT the driving force of science. We need to disprove theories, to learn where we are wrong. 

As long as we think that we are right, and do not learn that we are wrong, we do not move ahead.

\subsection{Complexity measures}

See Bennett.


41. Measures
411. Static measures: grading
412. Step counting
413. Classes
414. Indistinguishability

42. Hypothesis testing: Martin-Loef's significance testing

43. MDL
** Occam's razor:
** CAUSALITY AS SIMPLICITY: the simpler causes the more complex???

===> lies are more convincing than truths: 
===> androids will have a religion

44. INTENSIONALITY:
** bind causality to identity: trust
** recognize liars and not lies

45. Logical depth: time to evolve
** Why is the world complex? What pumps complexity? 
** Where does morphogenesis come from?


5. STRATIFIED CAUSALITY
** Hierarchies of causations
** Abstraction in sciences 
** SUBLIMATION in evolution: 

**** selfish modules carried by genomes 
****** distributed by viruses

**** selfish genes carried by individuals 
****** distributed through reproduction and selection

**** selfish individuals carried by societies
****** distributed through social economy and politics


6. UNIVERSAL COMPUTER = evaluator of strategies, speaker (translator) of a language

** an encodable mental function: there is a process called cognition

** if there is, then there is a fixed point
** it may not be able to decide: it has to clock out and randomize

** it consults oracles


\subsection{Computational consequences of evolution: Logical depth}
**** selection according to behaviors is undecidable
**** where decisions are needed
**** genes are not transferred not just horizontally (hypersex) but split into genomes
**** that is why horizontal gene transfer got obstructed

EVOLUTION INTO EUCARIOTS IS INTENSIONAL SELECTION, NOT BEHAVIORAL

34. MSRS Thm: TT is finitely approximable
**** open ended selection according to behaviors

35. ORACLES: 
** layered language generation: 
**** words: a-machines --- arbitrary!
**** sentences: a-machines or FSM --- simple, with stack memory
**** messages: o-machines --- feedback from conversation
**** protocols: o-machines --- extensive oracle interactions, run in parallel
**** contexts, narratives, experience, identity --- o-interactions, complexity degrees

36. ACTOR LOGIC








==> PICS/comp-caus-0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Apr 28 20:55:41 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="190" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,40);(50,40);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,95);(15,95);(15,70);(15,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,40);(0,40);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,40);(10,40);(10,15);(10,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,50);(110,50);(110,20);(110,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(190,40);(190,40);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,95);(175,95);(175,70);(175,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,40);(140,40);(190,40);(190,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,40);(165,40);(165,15);(165,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,20);(110,20);(140,20);(140,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(158.12,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(120,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,50);(110,50);(140,20);(140,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,55);(125,55);(125,35);(125,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(140,40);(140,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,95);(35,95);(35,70);(35,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,40);(40,40);(40,15);(40,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,40);(25,40);(25,15);(25,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(180,40);(180,40);(180,15);(180,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,40);(150,40);(150,15);(150,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(155,95);(155,95);(155,70);(155,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(126.25,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(157.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(190,110)
\psline[linewidth=0.75](0,70)(50,70)
\psline[linewidth=0.75](0,70)(0,40)
\psline[linewidth=0.75](50,40)(50,70)
\psline[linewidth=0.75](15,95)(15,70)
\rput(25,110){$\nameslang$}
\rput(25,0){$\inputt$}
\psline[linewidth=0.75](0,40)(50,40)
\psline[linewidth=0.75](10,40)(10,15)
\rput(25,55){\machine}
\psline[linewidth=0.75](110,70)(190,70)
\psline[linewidth=0.75](110,50)(110,20)
\psline[linewidth=0.75](190,40)(190,70)
\psline[linewidth=0.75](175,95)(175,70)
\rput(165,110){$\nameslang$}
\rput(165,0){$\inputt$}
\psline[linewidth=0.75](140,40)(190,40)
\psline[linewidth=0.75](165,40)(165,15)
\psline[linewidth=0.75](110,20)(140,20)
\rput(158.12,55){\universal}
\rput(120,27.5){\program}
\psline[linewidth=0.75](110,50)(140,20)
\psline[linewidth=0.75](125,55)(125,35)
\psline[linewidth=0.75](110,70)(140,40)
\psline[linewidth=0.75](35,95)(35,70)
\psline[linewidth=0.75](40,40)(40,15)
\psline[linewidth=0.75](25,40)(25,15)
\psline[linewidth=0.75](180,40)(180,15)
\psline[linewidth=0.75](150,40)(150,15)
\psline[linewidth=0.75](155,95)(155,70)
\rput[l](126.25,40){$\dee$}
\rput[r](147.5,15){$\ceeone$}
\rput[r](162.5,15){$\ceetwo$}
\rput[r](177.5,15){$\ceethree$}
\rput[l](157.5,95){$\eeone$}
\rput[l](177.5,95){$\eetwo$}
\rput[r](7.5,15){$\ceeone$}
\rput[r](22.5,15){$\ceetwo$}
\rput[r](37.5,15){$\ceethree$}
\rput[l](17.5,95){$\eeone$}
\rput[l](37.5,95){$\eetwo$}
\end{pspicture}


==> PICS/comp-caus-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Apr 29 06:50:25 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="190" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(190,40);(190,40);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,95);(175,95);(175,70);(175,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,40);(140,40);(190,40);(190,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,40);(165,40);(165,15);(165,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(158.12,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,55);(125,55);(125,15);(125,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(140,40);(140,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(180,40);(180,40);(180,15);(180,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,40);(150,40);(150,15);(150,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(155,95);(155,95);(155,70);(155,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\description$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(123.75,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(157.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(190,110)
\psline[linewidth=0.75](110,70)(190,70)
\psline[linewidth=0.75](190,40)(190,70)
\psline[linewidth=0.75](175,95)(175,70)
\rput(165,110){$\nameslang$}
\rput(165,0){$\inputt$}
\psline[linewidth=0.75](140,40)(190,40)
\psline[linewidth=0.75](165,40)(165,15)
\rput(158.12,55){\universal}
\psline[linewidth=0.75](125,55)(125,15)
\psline[linewidth=0.75](110,70)(140,40)
\psline[linewidth=0.75](180,40)(180,15)
\psline[linewidth=0.75](150,40)(150,15)
\psline[linewidth=0.75](155,95)(155,70)
\rput(125,0){$\description$}
\rput[r](123.75,15){$\dee$}
\rput[r](147.5,15){$\ceeone$}
\rput[r](162.5,15){$\ceetwo$}
\rput[r](177.5,15){$\ceethree$}
\rput[l](157.5,95){$\eeone$}
\rput[l](177.5,95){$\eetwo$}
\rput(0,110){\nothing}
\rput(0,0){\nothing}
\end{pspicture}


==> PICS/comp-caus-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Apr 28 21:03:37 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="190" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,40);(50,40);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,95);(15,95);(15,70);(15,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,40);(0,40);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,40);(10,40);(10,15);(10,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,95);(35,95);(35,70);(35,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,40);(40,40);(40,15);(40,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,40);(25,40);(25,15);(25,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,93.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,93.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(190,110)
\psline[linewidth=0.75](0,70)(50,70)
\psline[linewidth=0.75](0,70)(0,40)
\psline[linewidth=0.75](50,40)(50,70)
\psline[linewidth=0.75](15,95)(15,70)
\rput(25,110){$\nameslang$}
\rput(25,0){$\inputt$}
\psline[linewidth=0.75](0,40)(50,40)
\psline[linewidth=0.75](10,40)(10,15)
\rput(25,55){\machine}
\psline[linewidth=0.75](35,95)(35,70)
\psline[linewidth=0.75](40,40)(40,15)
\psline[linewidth=0.75](25,40)(25,15)
\rput(190,110){\nothing}
\rput(190,0){\nothing}
\rput[r](7.5,13.75){$\ceeone$}
\rput[r](22.5,13.75){$\ceetwo$}
\rput[r](37.5,13.75){$\ceethree$}
\rput[l](17.5,93.75){$\eeone$}
\rput[l](37.5,93.75){$\eetwo$}
\end{pspicture}


==> PICS/comp-caus.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Apr 28 20:57:11 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="190" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,40);(50,40);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,95);(15,95);(15,70);(15,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,40);(0,40);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,40);(10,40);(10,15);(10,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,50);(110,50);(110,20);(110,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(190,40);(190,40);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,95);(175,95);(175,70);(175,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,40);(140,40);(190,40);(190,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,40);(165,40);(165,15);(165,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,20);(110,20);(140,20);(140,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(158.12,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(120,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(85,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,50);(110,50);(140,20);(140,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,55);(125,55);(125,35);(125,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(140,40);(140,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,95);(35,95);(35,70);(35,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,40);(40,40);(40,15);(40,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,40);(25,40);(25,15);(25,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(180,40);(180,40);(180,15);(180,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,40);(150,40);(150,15);(150,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(155,95);(155,95);(155,70);(155,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(126.25,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(157.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(190,110)
\psline[linewidth=0.75](0,70)(50,70)
\psline[linewidth=0.75](0,70)(0,40)
\psline[linewidth=0.75](50,40)(50,70)
\psline[linewidth=0.75](15,95)(15,70)
\rput(25,110){$\nameslang$}
\rput(25,0){$\inputt$}
\psline[linewidth=0.75](0,40)(50,40)
\psline[linewidth=0.75](10,40)(10,15)
\rput(25,55){\machine}
\psline[linewidth=0.75](110,70)(190,70)
\psline[linewidth=0.75](110,50)(110,20)
\psline[linewidth=0.75](190,40)(190,70)
\psline[linewidth=0.75](175,95)(175,70)
\rput(165,110){$\nameslang$}
\rput(165,0){$\inputt$}
\psline[linewidth=0.75](140,40)(190,40)
\psline[linewidth=0.75](165,40)(165,15)
\psline[linewidth=0.75](110,20)(140,20)
\rput(158.12,55){\universal}
\rput(120,27.5){\program}
\rput(85,55){\EQLS}
\psline[linewidth=0.75](110,50)(140,20)
\psline[linewidth=0.75](125,55)(125,35)
\psline[linewidth=0.75](110,70)(140,40)
\psline[linewidth=0.75](35,95)(35,70)
\psline[linewidth=0.75](40,40)(40,15)
\psline[linewidth=0.75](25,40)(25,15)
\psline[linewidth=0.75](180,40)(180,15)
\psline[linewidth=0.75](150,40)(150,15)
\psline[linewidth=0.75](155,95)(155,70)
\rput[l](126.25,40){$\dee$}
\rput[r](147.5,15){$\ceeone$}
\rput[r](162.5,15){$\ceetwo$}
\rput[r](177.5,15){$\ceethree$}
\rput[l](157.5,95){$\eeone$}
\rput[l](177.5,95){$\eetwo$}
\rput[r](7.5,15){$\ceeone$}
\rput[r](22.5,15){$\ceetwo$}
\rput[r](37.5,15){$\ceethree$}
\rput[l](17.5,95){$\eeone$}
\rput[l](37.5,95){$\eetwo$}
\end{pspicture}


==> PICS/comp-part.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Apr 28 21:00:08 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-7.5" x-max="202.5" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(132.5,70);(132.5,70);(202.5,70);(202.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(202.5,40);(202.5,40);(202.5,70);(202.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(192.5,95);(192.5,95);(192.5,70);(192.5,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(181.25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(172.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(162.5,40);(162.5,40);(202.5,40);(202.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(172.5,40);(172.5,40);(172.5,15);(172.5,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(176.25,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(100,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(127.5,40);(127.5,40);(127.5,15);(127.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(112.5,55);(112.5,55);(142.5,25);(142.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(192.5,40);(192.5,40);(192.5,15);(192.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(152.5,25);(152.5,25);(152.5,15);(152.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(172.5,95);(172.5,95);(172.5,70);(172.5,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\descriptionn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(-7.5,70);(-7.5,70);(82.5,70);(82.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(82.5,40);(82.5,40);(82.5,70);(82.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(62.5,95);(62.5,95);(62.5,70);(62.5,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(52.5,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(52.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(22.5,40);(22.5,40);(82.5,40);(82.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(52.5,40);(52.5,40);(52.5,15);(52.5,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(46.25,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(7.5,55);(7.5,55);(7.5,15);(7.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(-7.5,70);(-7.5,70);(22.5,40);(22.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(72.5,40);(72.5,40);(72.5,15);(72.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(32.5,40);(32.5,40);(32.5,15);(32.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(42.5,95);(42.5,95);(42.5,70);(42.5,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\descriptionn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(142.5,25);(142.5,25);(162.5,25);(162.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(112.5,55);(112.5,55);(132.5,55);(132.5,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(132.5,55);(132.5,55);(162.5,25);(162.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(132.5,70);(132.5,70);(162.5,40);(162.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(147.5,55);(147.5,55);(147.5,40);(147.5,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(137.5,40)"
%	 text-rotation= "-45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\partial
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(51.25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(71.25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(195,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(151.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(171.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(191.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(148.75,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(202.5,110)
\psline[linewidth=0.75](132.5,70)(202.5,70)
\psline[linewidth=0.75](202.5,40)(202.5,70)
\psline[linewidth=0.75](192.5,95)(192.5,70)
\rput(181.25,110){$\nameslang$}
\rput(172.5,0){$\inputt$}
\psline[linewidth=0.75](162.5,40)(202.5,40)
\psline[linewidth=0.75](172.5,40)(172.5,15)
\rput(176.25,55){\universal}
\rput(100,55){\EQLS}
\psline[linewidth=0.75](127.5,40)(127.5,15)
\psline[linewidth=0.75](112.5,55)(142.5,25)
\psline[linewidth=0.75](192.5,40)(192.5,15)
\psline[linewidth=0.75](152.5,25)(152.5,15)
\psline[linewidth=0.75](172.5,95)(172.5,70)
\rput(127.5,0){$\descriptionn$}
\psline[linewidth=0.75](-7.5,70)(82.5,70)
\psline[linewidth=0.75](82.5,40)(82.5,70)
\psline[linewidth=0.75](62.5,95)(62.5,70)
\rput(52.5,110){$\nameslang$}
\rput(52.5,0){$\inputt$}
\psline[linewidth=0.75](22.5,40)(82.5,40)
\psline[linewidth=0.75](52.5,40)(52.5,15)
\rput(46.25,55){\universal}
\psline[linewidth=0.75](7.5,55)(7.5,15)
\psline[linewidth=0.75](-7.5,70)(22.5,40)
\psline[linewidth=0.75](72.5,40)(72.5,15)
\psline[linewidth=0.75](32.5,40)(32.5,15)
\psline[linewidth=0.75](42.5,95)(42.5,70)
\rput(7.5,0){$\descriptionn$}
\psline[linewidth=0.75](142.5,25)(162.5,25)
\psline[linewidth=0.75](112.5,55)(132.5,55)
\psline[linewidth=0.75](132.5,55)(162.5,25)
\psline[linewidth=0.75](132.5,70)(162.5,40)
\psline[linewidth=0.75](147.5,55)(147.5,40)
\rput{-45}(137.5,40){\partial}
\rput[r](5,15){$\dee$}
\rput[r](31.25,15){$\ceeone$}
\rput[r](51.25,15){$\ceetwo$}
\rput[r](71.25,15){$\ceethree$}
\rput[l](45,95){$\eeone$}
\rput[l](65,95){$\eetwo$}
\rput[l](175,95){$\eeone$}
\rput[l](195,95){$\eetwo$}
\rput[r](125,16.25){$\dee$}
\rput[r](151.25,16.25){$\ceeone$}
\rput[r](171.25,16.25){$\ceetwo$}
\rput[r](191.25,16.25){$\ceethree$}
\rput[l](148.75,43.75){$\dee$}
\end{pspicture}


==> PICS/comp.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 13 16:23:02 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,65);(20,65);(20,47.5);(20,47.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,71.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,22.5);(30,22.5);(30,7.5);(30,7.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,53.12);(70,53.12);(130,53.12);(130,53.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(70,16.25);(70,16.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,28.12);(130,28.12);(130,53.12);(130,53.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,65);(110,65);(110,53.12);(110,53.12)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,71.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,28.12);(95,28.12);(130,28.12);(130,28.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,28.12);(110,28.12);(110,7.5);(110,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,16.25);(70,16.25);(95,16.25);(95,16.25)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(108.12,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,23.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(95,16.25);(95,16.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(83.12,40);(83.12,40);(83.12,28.12);(83.12,28.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,53.12);(70,53.12);(95,28.12);(95,28.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,22.5);(10,22.5);(10,7.5);(10,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,15);(80,15);(80,7.5);(80,7.5)"
%	 stroke-width= "0.75"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,71.25)
\psline[linewidth=0.75](0,47.5)(40,47.5)
\psline[linewidth=0.75](0,47.5)(0,22.5)
\psline[linewidth=0.75](40,22.5)(40,47.5)
\psline[linewidth=0.75](20,65)(20,47.5)
\rput(20,71.25){$\nameslang$}
\rput(30,1.25){$\inputt$}
\psline[linewidth=0.75](0,22.5)(40,22.5)
\psline[linewidth=0.75](30,22.5)(30,7.5)
\rput(20,35){\machine}
\psline[linewidth=0.75](70,53.12)(130,53.12)
\psline[linewidth=0.75](70,41.25)(70,16.25)
\psline[linewidth=0.75](130,28.12)(130,53.12)
\psline[linewidth=0.75](110,65)(110,53.12)
\rput(110,71.25){$\nameslang$}
\rput(110,1.25){$\inputt$}
\psline[linewidth=0.75](95,28.12)(130,28.12)
\psline[linewidth=0.75](110,28.12)(110,7.5)
\psline[linewidth=0.75](70,16.25)(95,16.25)
\rput(108.12,40){\universal}
\rput(75,23.75){\program}
\rput(55,35){\EQLS}
\psline[linewidth=0.75](70,41.25)(95,16.25)
\psline[linewidth=0.75](83.12,40)(83.12,28.12)
\psline[linewidth=0.75](70,53.12)(95,28.12)
\psline[linewidth=0.75](10,22.5)(10,7.5)
\psline[linewidth=0.75](80,15)(80,7.5)
\end{pspicture}


==> PICS/computation-tight.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Apr 29 04:13:13 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="305" y-min="30" y-max="90" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,60);(100,60);(100,30);(100,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,60);(125,60);(125,30);(125,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(95,60);(95,60);(75,80);(75,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(75,80);(75,80);(130,80);(130,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(95,60);(95,60);(130,60);(130,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(130,80);(130,80);(130,60);(130,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,90);(110,90);(110,80);(110,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,70);(85,70);(85,57.5);(85,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(167.5,57.5);(167.5,57.5);(167.5,45);(167.5,45)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(185,47.5);(185,47.5);(185,30);(185,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(157.5,67.5);(157.5,67.5);(177.5,67.5);(177.5,67.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(197.5,47.5);(197.5,47.5);(177.5,47.5);(177.5,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(197.5,60);(197.5,60);(177.5,80);(177.5,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(177.5,67.5);(177.5,67.5);(197.5,47.5);(197.5,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(177.5,80);(177.5,80);(217.5,80);(217.5,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(187.5,70);(187.5,70);(187.5,57.5);(187.5,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(197.5,60);(197.5,60);(217.5,60);(217.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(217.5,80);(217.5,80);(217.5,60);(217.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(157.5,67.5);(157.5,67.5);(177.5,47.5);(177.5,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(197.5,90);(197.5,90);(197.5,80);(197.5,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(185,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(207.5,60);(207.5,60);(207.5,30);(207.5,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,57.5)"
%	 text-rotation= "-45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(203.75,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(97.5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(120,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(112.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(200,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(205,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(182.5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(110,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(157.5,55);(157.5,55);(157.5,35);(157.5,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(157.5,35);(157.5,35);(177.5,35);(177.5,35)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(157.5,55);(157.5,55);(177.5,35);(177.5,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(75,47.5);(75,47.5);(95,47.5);(95,47.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(82.5,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(75,67.5);(75,67.5);(95,47.5);(95,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(75,67.5);(75,67.5);(75,47.5);(75,47.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(82.5,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,60);(40,60);(40,30);(40,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,60);(0,60);(0,80);(0,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,80);(0,80);(50,80);(50,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,60);(0,60);(50,60);(50,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,80);(50,80);(50,60);(50,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,88.75);(25,88.75);(25,80);(25,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(7.5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(37.5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(27.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(25,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,60);(10,60);(10,30);(10,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(292.5,60);(292.5,60);(292.5,30);(292.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(245,47.5);(245,47.5);(245,67.5);(245,67.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(265,80);(265,80);(305,80);(305,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(285,60);(285,60);(305,60);(305,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(305,80);(305,80);(305,60);(305,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(287.5,90);(287.5,90);(287.5,80);(287.5,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(257.5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(290,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(290,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(260,47.5);(260,47.5);(260,30);(260,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(285,60);(285,60);(265,80);(265,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(245,47.5);(245,47.5);(285,47.5);(285,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(245,67.5);(245,67.5);(265,67.5);(265,67.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(285,47.5);(285,47.5);(265,67.5);(265,67.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(275,70);(275,70);(275,57.5);(275,57.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(272.5,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(233.75,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsc$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(63.75,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(291.25,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(258.75,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gx$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(305,90)
\psline[linewidth=0.75](100,60)(100,30)
\psline[linewidth=0.75](125,60)(125,30)
\psline[linewidth=0.75](95,60)(75,80)
\psline[linewidth=0.75](75,80)(130,80)
\psline[linewidth=0.75](95,60)(130,60)
\psline[linewidth=0.75](130,80)(130,60)
\psline[linewidth=0.75](110,90)(110,80)
\psline[linewidth=0.75](85,70)(85,57.5)
\psline[linewidth=0.75](167.5,57.5)(167.5,45)
\psline[linewidth=0.75](185,47.5)(185,30)
\psline[linewidth=0.75](157.5,67.5)(177.5,67.5)
\psline[linewidth=0.75](197.5,47.5)(177.5,47.5)
\psline[linewidth=0.75](197.5,60)(177.5,80)
\psline[linewidth=0.75](177.5,67.5)(197.5,47.5)
\psline[linewidth=0.75](177.5,80)(217.5,80)
\psline[linewidth=0.75](187.5,70)(187.5,57.5)
\psline[linewidth=0.75](197.5,60)(217.5,60)
\psline[linewidth=0.75](217.5,80)(217.5,60)
\psline[linewidth=0.75](157.5,67.5)(177.5,47.5)
\psline[linewidth=0.75](197.5,90)(197.5,80)
\rput[r](185,67.5){$\Progtype$}
\psline[linewidth=0.75](207.5,60)(207.5,30)
\rput{-45}(177.5,57.5){$\partial$}
\rput(203.75,70){$\universal$}
\rput[r](97.5,31.25){$\Progk$}
\rput[r](120,31.25){$\Progm$}
\rput[l](112.5,88.75){$\Progn$}
\rput[l](200,88.75){$\Progn$}
\rput[r](205,31.25){$\Progm$}
\rput[r](182.5,31.25){$\Progk$}
\rput(110,70){$\universalmkn$}
\psline[linewidth=0.75](157.5,55)(157.5,35)
\psline[linewidth=0.75](157.5,35)(177.5,35)
\rput(165,40){\program}
\psline[linewidth=0.75](157.5,55)(177.5,35)
\psline[linewidth=0.75](75,47.5)(95,47.5)
\rput(82.5,52.5){\program}
\psline[linewidth=0.75](75,67.5)(95,47.5)
\psline[linewidth=0.75](75,67.5)(75,47.5)
\rput[r](165,55){$\Progtype$}
\rput[r](82.5,67.5){$\Progtype$}
\psline[linewidth=0.75](40,60)(40,30)
\psline[linewidth=0.75](0,60)(0,80)
\psline[linewidth=0.75](0,80)(50,80)
\psline[linewidth=0.75](0,60)(50,60)
\psline[linewidth=0.75](50,80)(50,60)
\psline[linewidth=0.75](25,88.75)(25,80)
\rput[r](7.5,31.25){$\Progk$}
\rput[r](37.5,31.25){$\Progm$}
\rput[l](27.5,88.75){$\Progn$}
\rput(25,70){\gee}
\psline[linewidth=0.75](10,60)(10,30)
\psline[linewidth=0.75](292.5,60)(292.5,30)
\psline[linewidth=0.75](245,47.5)(245,67.5)
\psline[linewidth=0.75](265,80)(305,80)
\psline[linewidth=0.75](285,60)(305,60)
\psline[linewidth=0.75](305,80)(305,60)
\psline[linewidth=0.75](287.5,90)(287.5,80)
\rput[r](257.5,31.25){$\Progk$}
\rput[r](290,31.25){$\Progm$}
\rput[l](290,88.75){$\Progn$}
\psline[linewidth=0.75](260,47.5)(260,30)
\psline[linewidth=0.75](285,60)(265,80)
\psline[linewidth=0.75](245,47.5)(285,47.5)
\psline[linewidth=0.75](245,67.5)(265,67.5)
\psline[linewidth=0.75](285,47.5)(265,67.5)
\psline[linewidth=0.75](275,70)(275,57.5)
\rput[r](272.5,67.5){$\Progtype$}
\rput(145,70){$\eqlsb$}
\rput(233.75,70){$\eqlsc$}
\rput(63.75,70){$\eqlsa$}
\rput(291.25,70){$\universal$}
\rput(258.75,57.5){$\Gx$}
\end{pspicture}


==> PICS/curved.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 08 11:25:32 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="140" y-min="0" y-max="45" auto-bounding="true">
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 points= "(10,20);(10,20);(15,30);(20,25);(25,20);(25,0);
%	(35,10);(45,20);(55,20);(65,15);(75,10);(65,25);
%	(80,30);(95,35);(80,45);(100,45);(120,45);(105,45);
%	(120,40);(135,35);(125,45);(130,30);(135,15);(140,20);
%	(140,20);(140,20);(140,20);(140,20);(140,20);(140,20);
%	(140,20)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(140,45)
\pscustom[linewidth=0.4]{\psbezier(10,20)(10,20)(15,30)(20,25)
\psbezier(25,20)(25,0)(35,10)
\psbezier(45,20)(55,20)(65,15)
\psbezier(75,10)(65,25)(80,30)
\psbezier(95,35)(80,45)(100,45)
\psbezier(120,45)(105,45)(120,40)
\psbezier(135,35)(125,45)(130,30)
\psbezier(135,15)(140,20)(140,20)
\psbezier(140,20)(140,20)(140,20)
\psbezier(140,20)(140,20)(140,20)
}
\end{pspicture}


==> PICS/kleene-11.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Oct 25 15:24:50 GMT-05:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="13.75" x-max="173.75" y-min="-1.25" y-max="112.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(113.75,94.37);(113.75,94.37);(173.75,94.37);(173.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(113.75,60);(113.75,60);(113.75,35);(113.75,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(173.75,69.37);(173.75,69.37);(173.75,94.37);(173.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(153.75,106.25);(153.75,106.25);(153.75,94.37);(153.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(153.75,112.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165.62,-1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(138.75,69.37);(138.75,69.37);(173.75,69.37);(173.75,69.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,69.37);(165,69.37);(165,3.75);(165,3.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(113.75,35);(113.75,35);(138.75,35);(138.75,35)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(151.87,81.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(121.25,41.87)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(98.75,76.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(113.75,60);(113.75,60);(138.75,35);(138.75,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(126.25,81.88);(126.25,81.88);(126.25,48.12);(126.25,48.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(113.75,94.37);(113.75,94.37);(138.75,69.37);(138.75,69.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,94.38);(33.75,94.38);(83.75,94.37);(83.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(83.75,69.37);(83.75,69.37);(83.75,94.37);(83.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(58.75,106.25);(58.75,106.25);(58.75,94.37);(58.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(58.75,112.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(74.38,-1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(33.75,69.38);(33.75,69.38);(83.75,69.37);(83.75,69.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(73.75,69.37);(73.75,69.37);(73.75,3.75);(73.75,3.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(43.75,69.38);(43.75,69.38);(43.75,48.12);(43.75,48.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,94.38);(33.75,94.38);(33.75,69.38);(33.75,69.38)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(58.75,81.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(13.75,56.24);(13.75,56.24);(35,56.24);(35,56.24)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,36.25);(55,36.25);(33.75,36.25);(33.75,36.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,56.24);(35,56.24);(55,36.25);(55,36.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.75,56.24);(13.75,56.24);(33.75,36.25);(33.75,36.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(34.38,14.38);(34.38,14.38);(34.38,3.75);(34.38,3.75)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(35.78,12.96)"
%	 fill-style= "solid"
%	 p2= "(35.78,15.78)"
%	 fill-color= "#330033"
%	 p1= "(32.96,15.78)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,36.25);(45,36.25);(45,25);(45,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(24.38,45);(24.38,45);(24.38,23.76);(24.38,23.76)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,25);(45,25);(34.38,14.38);(34.38,14.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(24.38,23.76);(24.38,23.76);(34.38,13.75);(34.38,13.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,69.37);(145,69.37);(145,3.75);(145,3.75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(34.38,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<ellipse p3= "(127.81,45.94)"
%	 fill-style= "solid"
%	 p2= "(127.81,49.06)"
%	 p1= "(124.69,49.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(45.31,45.31)"
%	 fill-style= "solid"
%	 p2= "(45.31,48.44)"
%	 p1= "(42.19,48.44)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(173.75,112.5)
\psline[linewidth=0.75](113.75,94.37)(173.75,94.37)
\psline[linewidth=0.75](113.75,60)(113.75,35)
\psline[linewidth=0.75](173.75,69.37)(173.75,94.37)
\psline[linewidth=0.75](153.75,106.25)(153.75,94.37)
\rput(153.75,112.5){$\nameslang$}
\rput(165.62,-1.25){$\inputt$}
\psline[linewidth=0.75](138.75,69.37)(173.75,69.37)
\psline[linewidth=0.75](165,69.37)(165,3.75)
\psline[linewidth=0.75](113.75,35)(138.75,35)
\rput(151.87,81.25){\universal}
\rput(121.25,41.87){\program}
\rput(98.75,76.25){\EQLS}
\psline[linewidth=0.75](113.75,60)(138.75,35)
\psline[linewidth=0.75](126.25,81.88)(126.25,48.12)
\psline[linewidth=0.75](113.75,94.37)(138.75,69.37)
\psline[linewidth=0.75](33.75,94.38)(83.75,94.37)
\psline[linewidth=0.75](83.75,69.37)(83.75,94.37)
\psline[linewidth=0.75](58.75,106.25)(58.75,94.37)
\rput(58.75,112.5){$\nameslang$}
\rput(74.38,-1.25){$\inputt$}
\psline[linewidth=0.75](33.75,69.38)(83.75,69.37)
\psline[linewidth=0.75](73.75,69.37)(73.75,3.75)
\psline[linewidth=0.75](43.75,69.38)(43.75,48.12)
\psline[linewidth=0.75](33.75,94.38)(33.75,69.38)
\rput(58.75,81.25){$\gee$}
\psline[linewidth=0.75](13.75,56.24)(35,56.24)
\psline[linewidth=0.75](55,36.25)(33.75,36.25)
\psline[linewidth=0.75](35,56.24)(55,36.25)
\psline[linewidth=0.75](13.75,56.24)(33.75,36.25)
\psline[linewidth=0.75](34.38,14.38)(34.38,3.75)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(34.37,14.37){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](45,36.25)(45,25)
\psline[linewidth=0.75](24.38,45)(24.38,23.76)
\psline[linewidth=0.75](45,25)(34.38,14.38)
\psline[linewidth=0.75](24.38,23.76)(34.38,13.75)
\psline[linewidth=0.75](145,69.37)(145,3.75)
\rput(145,-0.62){$\progtype$}
\rput(34.38,-1.25){$\progtype$}
\rput(35,45){$\parteval$}
\rput{0}(126.25,47.5){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(43.75,46.88){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\end{pspicture}


==> PICS/kleene-21.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Oct 25 15:38:19 GMT-05:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="368.75" y-min="0.62" y-max="131.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(125,113.12);(125,113.12);(185,113.12);(185,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,78.75);(125,78.75);(125,53.75);(125,53.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,88.12);(185,88.12);(185,113.12);(185,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,125);(165,125);(165,113.12);(165,113.12)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,131.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(176.25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,88.12);(150,88.12);(185,88.12);(185,88.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(176.25,88.12);(176.25,88.12);(176.25,7.5);(176.25,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,53.75);(125,53.75);(150,53.75);(150,53.75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(163.12,100)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(132.5,60.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,95)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,78.75);(125,78.75);(150,53.75);(150,53.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,100.62);(137.5,100.62);(137.5,66.88);(137.5,66.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,113.12);(125,113.12);(150,88.12);(150,88.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,113.12);(45,113.12);(95,113.12);(95,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,88.12);(95,88.12);(95,113.12);(95,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,125);(70,125);(70,113.12);(70,113.12)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,131.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,88.12);(45,88.12);(95,88.12);(95,88.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,88.12);(85,88.12);(85,6.88);(85,6.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,88.12);(55,88.12);(55,66.87);(55,66.87)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,113.12);(45,113.12);(45,88.12);(45,88.12)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,75);(25,75);(46.25,75);(46.25,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(66.25,55);(66.25,55);(45,55);(45,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.25,75);(46.25,75);(66.25,55);(66.25,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,75);(25,75);(45,55);(45,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45.62,33.12);(45.62,33.12);(45.62,22.5);(45.62,22.5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(47.04,31.72)"
%	 fill-style= "solid"
%	 p2= "(47.04,34.54)"
%	 fill-color= "#330033"
%	 p1= "(44.22,34.54)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.25,55);(56.25,55);(56.25,43.75);(56.25,43.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35.62,63.75);(35.62,63.75);(35.62,42.5);(35.62,42.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.25,43.75);(56.25,43.75);(45.62,33.12);(45.62,33.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35.62,42.5);(35.62,42.5);(45.62,32.5);(45.62,32.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(156.25,88.12);(156.25,88.12);(156.25,22.5);(156.25,22.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,33.75);(35,33.75);(35,8.75);(35,8.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,8.75);(35,8.75);(60,8.75);(60,8.75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,15.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,33.75);(35,33.75);(60,8.75);(60,8.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(144.38,34.38);(144.38,34.38);(144.38,9.38);(144.38,9.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(144.38,9.38);(144.38,9.38);(169.38,9.38);(169.38,9.38)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(151.88,16.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(144.38,34.38);(144.38,34.38);(169.38,9.38);(169.38,9.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215.62,112.5);(215.62,112.5);(275.62,112.5);(275.62,112.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275.62,87.5);(275.62,87.5);(275.62,112.5);(275.62,112.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255.62,124.38);(255.62,124.38);(255.62,112.5);(255.62,112.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(255.62,130.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(266.88,0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(240.62,87.5);(240.62,87.5);(275.62,87.5);(275.62,87.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(266.88,87.5);(266.88,87.5);(266.88,6.88);(266.88,6.88)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(253.74,99.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(200.62,94.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(215.62,112.5);(215.62,112.5);(240.62,87.5);(240.62,87.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(237.5,35);(237.5,35);(237.5,24.38);(237.5,24.38)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(238.91,33.59)"
%	 fill-style= "solid"
%	 p2= "(238.91,36.41)"
%	 fill-color= "#330033"
%	 p1= "(236.09,36.41)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(248.12,87.5);(248.12,87.5);(248.12,45.62);(248.12,45.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(227.5,100.62);(227.5,100.62);(227.5,44.38);(227.5,44.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(248.12,45.62);(248.12,45.62);(237.5,35);(237.5,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(227.5,44.38);(227.5,44.38);(237.5,34.38);(237.5,34.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(226.88,35.62);(226.88,35.62);(226.88,10.62);(226.88,10.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(226.88,10.62);(226.88,10.62);(251.88,10.62);(251.88,10.62)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(234.38,17.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(226.88,35.62);(226.88,35.62);(251.88,10.62);(251.88,10.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315.62,113.12);(315.62,113.12);(368.75,113.12);(368.75,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(368.75,88.12);(368.75,88.12);(368.75,113.12);(368.75,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(343.75,125);(343.75,125);(343.75,113.12);(343.75,113.12)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(343.75,131.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(358.75,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(340.62,88.12);(340.62,88.12);(368.75,88.12);(368.75,88.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(358.75,88.12);(358.75,88.12);(358.75,6.88);(358.75,6.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(328.75,99.38);(328.75,99.38);(328.75,66.87);(328.75,66.87)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315.62,113.12);(315.62,113.12);(340.62,88.12);(340.62,88.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(298.75,75);(298.75,75);(320,75);(320,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,55);(340,55);(318.75,55);(318.75,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,75);(320,75);(340,55);(340,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(298.75,75);(298.75,75);(318.75,55);(318.75,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(319.38,33.12);(319.38,33.12);(319.38,22.5);(319.38,22.5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(320.78,31.72)"
%	 fill-style= "solid"
%	 p2= "(320.78,34.54)"
%	 fill-color= "#330033"
%	 p1= "(317.97,34.54)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,55);(330,55);(330,43.75);(330,43.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(309.38,63.75);(309.38,63.75);(309.38,42.5);(309.38,42.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,43.75);(330,43.75);(319.38,33.12);(319.38,33.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(309.38,42.5);(309.38,42.5);(319.38,32.5);(319.38,32.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(308.75,33.75);(308.75,33.75);(308.75,8.75);(308.75,8.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(308.75,8.75);(308.75,8.75);(333.75,8.75);(333.75,8.75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(316.25,15.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(308.75,33.75);(308.75,33.75);(333.75,8.75);(333.75,8.75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(350.62,100.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(291.88,95)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(44.38,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(319.38,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<ellipse p3= "(139.06,64.69)"
%	 fill-style= "solid"
%	 p2= "(139.06,67.81)"
%	 p1= "(135.94,67.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(56.41,64.22)"
%	 fill-style= "solid"
%	 p2= "(56.41,67.04)"
%	 fill-color= "#330033"
%	 p1= "(53.59,67.04)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(157.81,20.94)"
%	 fill-style= "solid"
%	 p2= "(157.81,24.06)"
%	 p1= "(154.69,24.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(239.06,23.44)"
%	 fill-style= "solid"
%	 p2= "(239.06,26.56)"
%	 p1= "(235.94,26.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(330.16,64.84)"
%	 fill-style= "solid"
%	 p2= "(330.16,67.66)"
%	 fill-color= "#330033"
%	 p1= "(327.34,67.66)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(47.18,20.94)"
%	 fill-style= "solid"
%	 p2= "(47.18,24.06)"
%	 p1= "(44.06,24.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(320.94,21.56)"
%	 fill-style= "solid"
%	 p2= "(320.94,24.69)"
%	 p1= "(317.82,24.69)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,80);(295,80);(322.5,80);(322.5,80);(322.5,80);(347.5,55);
%	(347.5,55);(347.5,55);(347.5,5);(347.5,5);(347.5,5);(295,5);
%	(295,5);(295,5);(295,5);(295,5);(295,5);(295,80)"
%	 stroke-color= "#cc0033"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(47.5,80);(47.5,80);(47.5,80);(72.5,55);
%	(72.5,55);(72.5,55);(72.5,5);(72.5,5);(72.5,5);(20,5);
%	(20,5);(20,5);(20,5);(20,5);(20,5);(20,80)"
%	 stroke-color= "#cc0033"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(368.75,131.25)
\psline[linewidth=0.75](125,113.12)(185,113.12)
\psline[linewidth=0.75](125,78.75)(125,53.75)
\psline[linewidth=0.75](185,88.12)(185,113.12)
\psline[linewidth=0.75](165,125)(165,113.12)
\rput(165,131.25){$\nameslang$}
\rput(176.25,1.25){$\inputt$}
\psline[linewidth=0.75](150,88.12)(185,88.12)
\psline[linewidth=0.75](176.25,88.12)(176.25,7.5)
\psline[linewidth=0.75](125,53.75)(150,53.75)
\rput(163.12,100){\universal}
\rput(132.5,60.62){\program}
\rput(110,95){\EQLS}
\psline[linewidth=0.75](125,78.75)(150,53.75)
\psline[linewidth=0.75](137.5,100.62)(137.5,66.88)
\psline[linewidth=0.75](125,113.12)(150,88.12)
\psline[linewidth=0.75](45,113.12)(95,113.12)
\psline[linewidth=0.75](95,88.12)(95,113.12)
\psline[linewidth=0.75](70,125)(70,113.12)
\rput(70,131.25){$\nameslang$}
\rput(85,1.25){$\inputt$}
\psline[linewidth=0.75](45,88.12)(95,88.12)
\psline[linewidth=0.75](85,88.12)(85,6.88)
\psline[linewidth=0.75](55,88.12)(55,66.87)
\psline[linewidth=0.75](45,113.12)(45,88.12)
\rput(70,100){$\gee$}
\psline[linewidth=0.75](25,75)(46.25,75)
\psline[linewidth=0.75](66.25,55)(45,55)
\psline[linewidth=0.75](46.25,75)(66.25,55)
\psline[linewidth=0.75](25,75)(45,55)
\psline[linewidth=0.75](45.62,33.12)(45.62,22.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(45.63,33.13){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](56.25,55)(56.25,43.75)
\psline[linewidth=0.75](35.62,63.75)(35.62,42.5)
\psline[linewidth=0.75](56.25,43.75)(45.62,33.12)
\psline[linewidth=0.75](35.62,42.5)(45.62,32.5)
\psline[linewidth=0.75](156.25,88.12)(156.25,22.5)
\psline[linewidth=0.75](35,33.75)(35,8.75)
\psline[linewidth=0.75](35,8.75)(60,8.75)
\rput(42.5,15.62){\program}
\psline[linewidth=0.75](35,33.75)(60,8.75)
\psline[linewidth=0.75](144.38,34.38)(144.38,9.38)
\psline[linewidth=0.75](144.38,9.38)(169.38,9.38)
\rput(151.88,16.25){\program}
\psline[linewidth=0.75](144.38,34.38)(169.38,9.38)
\psline[linewidth=0.75](215.62,112.5)(275.62,112.5)
\psline[linewidth=0.75](275.62,87.5)(275.62,112.5)
\psline[linewidth=0.75](255.62,124.38)(255.62,112.5)
\rput(255.62,130.62){$\nameslang$}
\rput(266.88,0.62){$\inputt$}
\psline[linewidth=0.75](240.62,87.5)(275.62,87.5)
\psline[linewidth=0.75](266.88,87.5)(266.88,6.88)
\rput(253.74,99.38){\universal}
\rput(200.62,94.38){\EQLS}
\psline[linewidth=0.75](215.62,112.5)(240.62,87.5)
\psline[linewidth=0.75](237.5,35)(237.5,24.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(237.5,35){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](248.12,87.5)(248.12,45.62)
\psline[linewidth=0.75](227.5,100.62)(227.5,44.38)
\psline[linewidth=0.75](248.12,45.62)(237.5,35)
\psline[linewidth=0.75](227.5,44.38)(237.5,34.38)
\psline[linewidth=0.75](226.88,35.62)(226.88,10.62)
\psline[linewidth=0.75](226.88,10.62)(251.88,10.62)
\rput(234.38,17.5){\program}
\psline[linewidth=0.75](226.88,35.62)(251.88,10.62)
\psline[linewidth=0.75](315.62,113.12)(368.75,113.12)
\psline[linewidth=0.75](368.75,88.12)(368.75,113.12)
\psline[linewidth=0.75](343.75,125)(343.75,113.12)
\rput(343.75,131.25){$\nameslang$}
\rput(358.75,1.25){$\inputt$}
\psline[linewidth=0.75](340.62,88.12)(368.75,88.12)
\psline[linewidth=0.75](358.75,88.12)(358.75,6.88)
\psline[linewidth=0.75](328.75,99.38)(328.75,66.87)
\psline[linewidth=0.75](315.62,113.12)(340.62,88.12)
\psline[linewidth=0.75](298.75,75)(320,75)
\psline[linewidth=0.75](340,55)(318.75,55)
\psline[linewidth=0.75](320,75)(340,55)
\psline[linewidth=0.75](298.75,75)(318.75,55)
\psline[linewidth=0.75](319.38,33.12)(319.38,22.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(319.38,33.13){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.4)}
\psline[linewidth=0.75](330,55)(330,43.75)
\psline[linewidth=0.75](309.38,63.75)(309.38,42.5)
\psline[linewidth=0.75](330,43.75)(319.38,33.12)
\psline[linewidth=0.75](309.38,42.5)(319.38,32.5)
\psline[linewidth=0.75](308.75,33.75)(308.75,8.75)
\psline[linewidth=0.75](308.75,8.75)(333.75,8.75)
\rput(316.25,15.62){\program}
\psline[linewidth=0.75](308.75,33.75)(333.75,8.75)
\rput(350.62,100.62){\universal}
\rput(291.88,95){\EQLS}
\rput(44.38,65){$\parteval$}
\rput(319.38,65){$\parteval$}
\rput{0}(137.5,66.25){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(55,65.63){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\rput{0}(156.25,22.5){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(237.5,25){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(328.75,66.25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\rput{0}(45.62,22.5){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{90}(319.38,23.12){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\newrgbcolor{userLineColour}{0.8 0 0.2}
\pscustom[linewidth=0.45,linecolor=userLineColour]{\psline(295,80)(322.5,80)
\psline(322.5,80)(347.5,55)
\psline(347.5,55)(347.5,5)
\psline(347.5,5)(295,5)
\psbezier(295,5)(295,5)(295,5)
\psline(295,5)(295,80)
\closepath}
\rput(335,25){$\Gee$}
\newrgbcolor{userLineColour}{0.8 0 0.2}
\pscustom[linewidth=0.45,linecolor=userLineColour]{\psline(20,80)(47.5,80)
\psline(47.5,80)(72.5,55)
\psline(72.5,55)(72.5,5)
\psline(72.5,5)(20,5)
\psbezier(20,5)(20,5)(20,5)
\psline(20,5)(20,80)
\closepath}
\rput(60,25){$\Gee$}
\end{pspicture}


==> PICS/process-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 13 14:14:12 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="60" y-min="10" y-max="70" auto-bounding="true">
%<multicurve fill-style= "solid"
%	 arrow-head-inset-scale= "0"
%	 fill-color= "#999999"
%	 points= "(5,36.25);(5,36.25);(5,15);(5,15)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 arrow-head-inset-scale= "0"
%	 fill-color= "#999999"
%	 points= "(5,60);(5,60);(5,40);(5,40)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 arrow-head-inset-scale= "0"
%	 fill-color= "#999999"
%	 points= "(8.75,36.25);(8.75,36.25);(30,15);(30,15)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 arrow-head-inset-scale= "0"
%	 fill-color= "#999999"
%	 points= "(33.75,36.25);(33.75,36.25);(55,15);(55,15)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 arrow-head-inset-scale= "0"
%	 fill-color= "#999999"
%	 points= "(30,60);(30,60);(30,45);(30,45)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 arrow-head-inset-scale= "0"
%	 fill-color= "#999999"
%	 points= "(25,40);(25,40);(5,40);(5,40)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<ellipse p3= "(10,35)"
%	 fill-style= "solid"
%	 p2= "(10,45)"
%	 fill-color= "#999999"
%	 p1= "(0,45)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(35,35)"
%	 fill-style= "solid"
%	 p2= "(35,45)"
%	 fill-color= "#999999"
%	 p1= "(25,45)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(10,60)"
%	 fill-style= "solid"
%	 p2= "(10,70)"
%	 fill-color= "#999999"
%	 p1= "(0,70)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(35,60)"
%	 fill-style= "solid"
%	 p2= "(35,70)"
%	 fill-color= "#999999"
%	 p1= "(25,70)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(10,10)"
%	 fill-style= "solid"
%	 p2= "(10,20)"
%	 fill-color= "#999999"
%	 p1= "(0,20)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(60,10)"
%	 fill-style= "solid"
%	 p2= "(60,20)"
%	 fill-color= "#999999"
%	 p1= "(50,20)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(35,10)"
%	 fill-style= "solid"
%	 p2= "(35,20)"
%	 fill-color= "#999999"
%	 p1= "(25,20)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(60,70)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid,arrowlength=1.5,arrowinset=0]{<-}(5,36.25)(5,15)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid,arrowlength=1.5,arrowinset=0]{<-}(5,60)(5,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid,arrowlength=1.5,arrowinset=0]{<-}(8.75,36.25)(30,15)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid,arrowlength=1.5,arrowinset=0]{<-}(33.75,36.25)(55,15)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid,arrowlength=1.5,arrowinset=0]{<-}(30,60)(30,45)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid,arrowlength=1.5,arrowinset=0]{<-}(25,40)(5,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(5,40){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(30,40){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(5,65){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(30,65){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(5,15){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(55,15){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(30,15){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\end{pspicture}


==> PICS/process-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 13 16:17:43 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="35" y-min="10" y-max="70" auto-bounding="true">
%<multicurve fill-style= "solid"
%	 arrow-head-inset-scale= "0"
%	 fill-color= "#999999"
%	 points= "(5,36.25);(5,36.25);(5,15);(5,15)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 arrow-head-inset-scale= "0"
%	 fill-color= "#999999"
%	 points= "(30,35);(30,35);(30,15);(30,15)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 arrow-head-inset-scale= "0"
%	 fill-color= "#999999"
%	 points= "(30,60);(30,60);(30,45);(30,45)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 arrow-head-inset-scale= "0"
%	 fill-color= "#999999"
%	 points= "(25,40);(25,40);(5,40);(5,40)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<ellipse p3= "(10,35)"
%	 fill-style= "solid"
%	 p2= "(10,45)"
%	 fill-color= "#999999"
%	 p1= "(0,45)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(35,35)"
%	 fill-style= "solid"
%	 p2= "(35,45)"
%	 fill-color= "#999999"
%	 p1= "(25,45)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(35,60)"
%	 fill-style= "solid"
%	 p2= "(35,70)"
%	 fill-color= "#999999"
%	 p1= "(25,70)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(10,10)"
%	 fill-style= "solid"
%	 p2= "(10,20)"
%	 fill-color= "#999999"
%	 p1= "(0,20)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(35,10)"
%	 fill-style= "solid"
%	 p2= "(35,20)"
%	 fill-color= "#999999"
%	 p1= "(25,20)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#999999"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(35,70)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid,arrowlength=1.5,arrowinset=0]{<-}(5,36.25)(5,15)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid,arrowlength=1.5,arrowinset=0]{<-}(30,35)(30,15)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid,arrowlength=1.5,arrowinset=0]{<-}(30,60)(30,45)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid,arrowlength=1.5,arrowinset=0]{<-}(25,40)(5,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(5,40){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(30,40){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(30,65){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(5,15){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\rput{0}(30,15){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(5,-5)}
\end{pspicture}


==> PICS/process-test.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 13 18:09:13 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="240" y-min="0" y-max="142.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(25,50);(25,50);(25,0);(25,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputtt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,50);(65,50);(65,0);(65,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(65,142.5);(65,142.5);(65,100);(65,100)"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<parallelogram p3= "(55,55)"
%	 fill-style= "none"
%	 p2= "(55,70)"
%	 p1= "(5,70)"
%	 stroke-color= "#999999"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(85,80)"
%	 fill-style= "none"
%	 p2= "(85,93.75)"
%	 p1= "(35,93.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(45,80);(45,80);(45,70);(45,70)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(68.12,134.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\outputtt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\inputt
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,100);(150,100);(240,100);(240,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,75);(150,75);(150,25);(150,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,50);(200,50);(240,50);(240,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,25);(150,25);(200,25);(200,25)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(190,28.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(122.5,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(175,25);(175,25);(175,0);(175,0)"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputtt$
%</text>
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(215,50);(215,50);(215,0);(215,0)"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(215,142.5);(215,142.5);(215,100);(215,100)"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(218.12,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\outputtt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(212.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\inputt
%</text>
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(25,55);(25,55);(25,50);(25,50)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(65,80);(65,80);(65,50);(65,50)"
%	 stroke-color= "#999999"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.75"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,100);(65,100);(65,93.75);(65,93.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(90,50)"
%	 fill-style= "none"
%	 p2= "(90,100)"
%	 p1= "(0,100)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160.62,41.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\graph
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,75);(150,75);(200,25);(200,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,75);(175,75);(175,50);(175,50)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(3.12,96.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\plann$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(216.88,75.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\lab
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,100);(150,100);(200,50);(200,50)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(168.75,97.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(240,50);(240,50);(240,100);(240,100)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,65.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\Language
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(240,142.5)
\psline[linewidth=0.75](25,50)(25,0)
\rput[r](22.5,5){$\inputtt$}
\psline[linewidth=0.75](65,50)(65,0)
\psline[linewidth=0.75,arrowlength=1.5,arrowinset=0]{<-}(65,142.5)(65,100)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\pspolygon[linewidth=0.75,linecolor=userLineColour](5,70)(55,70)(55,55)(5,55)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\pspolygon[linewidth=0.75,linecolor=userLineColour](35,93.75)(85,93.75)(85,80)(35,80)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,arrowlength=1.5,arrowinset=0]{<-}(45,80)(45,70)
\rput[l](68.12,134.38){\outputtt}
\rput[r](62.5,5){\inputt}
\psline[linewidth=0.75](150,100)(240,100)
\psline[linewidth=0.75](150,75)(150,25)
\psline[linewidth=0.75](200,50)(240,50)
\psline[linewidth=0.75](150,25)(200,25)
\rput[br](190,28.75){\program}
\rput(122.5,70){\EQLS}
\psline[linewidth=0.75,arrowlength=1.5,arrowinset=0]{<-}(175,25)(175,0)
\rput[r](172.5,5){$\inputtt$}
\psline[linewidth=0.75,arrowlength=1.5,arrowinset=0]{<-}(215,50)(215,0)
\psline[linewidth=0.75,arrowlength=1.5,arrowinset=0]{<-}(215,142.5)(215,100)
\rput[l](218.12,135){\outputtt}
\rput[r](212.5,5){\inputt}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,arrowlength=1.5,arrowinset=0]{<-}(25,55)(25,50)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour,arrowlength=1.5,arrowinset=0]{<-}(65,80)(65,50)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=0.75,linecolor=userLineColour](65,100)(65,93.75)
\pspolygon[linewidth=0.75](0,100)(90,100)(90,50)(0,50)
\rput(160.62,41.25){\graph}
\psline[linewidth=0.75](150,75)(200,25)
\psline[linewidth=0.75](175,75)(175,50)
\rput[tl](3.12,96.88){$\plann$}
\rput(216.88,75.62){\lab}
\psline[linewidth=0.75](150,100)(200,50)
\rput[tl](168.75,97.5){\universal}
\psline[linewidth=0.75](240,50)(240,100)
\rput[r](172.5,65.62){\Language}
\end{pspicture}


==> PICS/straight.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 08 11:27:50 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="140" y-min="8" y-max="45" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\top
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,8)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\bottom
%</text>
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(10,20);(10,20);(140,20);(140,20)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(140,45)
\rput(100,45){\top}
\rput(30,8){\bottom}
\psline[linewidth=0.45](10,20)(140,20)
\end{pspicture}


==> PICS/strings-0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Oct 23 15:34:50 GMT-05:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="52.5" y-min="-1.88" y-max="85" auto-bounding="true">
%<ellipse p3= "(24.06,78.44)"
%	 fill-style= "solid"
%	 p2= "(24.06,81.56)"
%	 p1= "(20.94,81.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,55);(7.5,55);(17.5,55);(17.5,55);(17.5,55);(12.5,50);
%	(12.5,50);(12.5,50);(7.5,55);(7.5,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(22.5,75);(22.5,75);(22.5,81.25);(22.5,81.25)"
%	 />
%<parallelogram p3= "(52.5,70)"
%	 fill-style= "none"
%	 p2= "(52.5,75)"
%	 p1= "(7.5,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,65);(12.5,65);(12.5,70);(12.5,70)"
%	 />
%<parallelogram p3= "(51.25,60)"
%	 fill-style= "none"
%	 p2= "(51.25,65)"
%	 p1= "(43.75,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,50);(32.5,50);(32.5,70);(32.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,35);(37.5,35);(37.5,70);(37.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,65);(47.5,65);(47.5,70);(47.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,45);(47.5,45);(47.5,60);(47.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,35);(37.5,35);(47.5,45);(47.5,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,35);(17.5,35);(32.5,50);(32.5,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1"
%	 points= "(22.5,50);(22.5,50);(37.5,35);(37.5,35)"
%	 stroke-overstrike= "true"
%	 />
%<ellipse p3= "(39.06,33.44)"
%	 fill-style= "solid"
%	 p2= "(39.06,36.56)"
%	 p1= "(35.94,36.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<parallelogram p3= "(25,60)"
%	 fill-style= "none"
%	 p2= "(25,65)"
%	 p1= "(0,65)"
%	 />
%<ellipse p3= "(19.06,33.44)"
%	 fill-style= "solid"
%	 p2= "(19.06,36.56)"
%	 p1= "(15.94,36.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,50);(2.5,50);(17.5,35);(17.5,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,50);(2.5,50);(2.5,60);(2.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(22.5,50);(22.5,50);(22.5,60);(22.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,75);(37.5,75);(37.5,83.75);(37.5,83.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,25);(17.5,25);(17.5,35);(17.5,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,5);(17.5,5);(37.5,25);(37.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,25);(37.5,25);(37.5,35);(37.5,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1"
%	 points= "(17.5,25);(17.5,25);(37.5,5);(37.5,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,0);(37.5,0);(37.5,5);(37.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,0);(17.5,0);(17.5,5);(17.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,55);(12.5,55);(12.5,60);(12.5,60)"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(52.5,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\northeast
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(0,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\northwest
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fun$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eich$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,53.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.88,3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.88,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ah$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(17.5,-1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(37.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.88,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Eee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(52.5,85)
\rput{90}(22.5,80){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(7.5,55)
(17.5,55)
(12.5,50)(7.5,55)
\psline(22.5,75)(22.5,81.25)
\pspolygon[](7.5,75)(52.5,75)(52.5,70)(7.5,70)
\psline(12.5,65)(12.5,70)
\pspolygon[](43.75,65)(51.25,65)(51.25,60)(43.75,60)
\psline(32.5,50)(32.5,70)
\psline(37.5,35)(37.5,70)
\psline(47.5,65)(47.5,70)
\psline(47.5,45)(47.5,60)
\psline(37.5,35)(47.5,45)
\psline(17.5,35)(32.5,50)
\psline[border=1](22.5,50)(37.5,35)
\rput{0}(37.5,35){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\pspolygon[](0,65)(25,65)(25,60)(0,60)
\rput{0}(17.5,35){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(2.5,50)(17.5,35)
\psline(2.5,50)(2.5,60)
\psline(22.5,50)(22.5,60)
\psline(37.5,75)(37.5,83.75)
\psline(17.5,25)(17.5,35)
\psline(17.5,5)(37.5,25)
\psline(37.5,25)(37.5,35)
\psline[border=1](17.5,25)(37.5,5)
\psline(37.5,0)(37.5,5)
\psline(17.5,0)(17.5,5)
\psline(12.5,55)(12.5,60)
\rput[tr](52.5,85){\northeast}
\rput[tl](0,85){\northwest}
\rput(47.5,62.5){$\gee$}
\rput(12.5,62.5){$\fun$}
\rput(30,72.5){$\eich$}
\rput(12.5,53.12){$\zero$}
\rput[r](16.88,3.12){$\Ah$}
\rput[r](36.88,3.12){$\Bee$}
\rput[r](16.88,30){$\Bee$}
\rput[r](36.88,30){$\Ah$}
\rput[t](17.5,-1.88){$\eex$}
\rput[t](37.5,-1.25){$\why$}
\rput[r](36.88,78.75){$\Eee$}
\end{pspicture}

